Adaptive Quantum Optimized Centroid Initialization

Prototype-based clustering algorithms such as k-means are sensitive to the selection of initial cluster centroids, with poor initialization leading to slower convergence and suboptimal solutions trapped in local minima. We present Adaptive Quantum Optimized Centroid Initialization (AQOCI), a method that formulates the centroid initialization problem as a Quadratic Unconstrained Binary Optimization (QUBO) problem and solves it using quantum annealing or quantum-inspired solvers. AQOCI extends a prior method (QOCI) by introducing an iterative refinement mechanism inspired by the Gauss-Seidel and Jacobi methods, enabling the recovery of real-valued centroid coordinates from binary solver outputs through adaptive scaling and offset adjustments. We evaluate AQOCI using three solver backends: TABU search, simulated annealing, and D-Wave's HybridBQM on synthetic Gaussian data with controlled sweeps over cluster separation, cluster count, dimensionality, and sample size, as well as on the MOTIF malware classification dataset, comparing against standard k-means with random initialization and k-means++ initialization. On the MOTIF dataset, AQOCI produces clusterings that are competitive with and, at smaller sample sizes, superior to k-means++, with V-measure improvements of up to 26\%. On synthetic data with heavily overlapping clusters, AQOCI--SimAnn outperforms k-means++ in V-measure. On well-separated synthetic data, k-means++ is clearly superior, and AQOCI exhibits a consistent performance plateau attributable to the binary encoding resolution. The dimensionality sweep demonstrates scalability to at least $d = 10$ without degradation.

==> guassian-tikz.tex <==

\begin{figure}[!t]
\centering
\begin{subfigure}[t]{0.485\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
    width=\linewidth,
    height=6.5cm,
    xlabel={Samples},
    ylabel={V-Measure},
    xmin=15, xmax=260,
    ymin=0.1, ymax=0.95,
    xtick={20,50,100,150,200,250},
    grid=major,
    grid style={gray!30},
    tick label style={font=\small},
    label style={font=\small},
    title={\small (a) V-Measure},
]
\addplot[color=clrRandom, mark=square*, thick, mark size=2pt]
    coordinates {(20,0.499)(30,0.270)(35,0.276)(40,0.368)
                 (45,0.468)(50,0.431)(100,0.238)(250,0.318)};
\addplot[color=clrTabu, mark=triangle*, thick, mark size=2pt]
    coordinates {(20,0.376)(30,0.254)(35,0.201)(40,0.227)
                 (45,0.414)(50,0.392)(100,0.188)(250,0.300)};
\addplot[color=clrSim, mark=diamond*, thick, mark size=2pt]
    coordinates {(20,0.376)(30,0.297)(35,0.276)(40,0.227)
                 (45,0.414)(50,0.392)(100,0.238)(250,0.300)};
\addplot[color=clrHybrid, mark=pentagon*, thick, mark size=2pt]
    coordinates {(20,0.376)(30,0.254)(35,0.223)(40,0.227)
                 (45,0.414)(50,0.392)(100,0.253)(250,0.316)};
\addplot[color=clrKpp, mark=o, thick, dashed, mark size=2pt]
    coordinates {(20,0.869)(30,0.744)(35,0.767)(40,0.704)
                 (45,0.775)(50,0.792)(100,0.770)(250,0.779)};
\end{axis}
\end{tikzpicture}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.485\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
    width=\linewidth,
    height=6.5cm,
    xlabel={Samples},
    ylabel={Silhouette Score},
    xmin=15, xmax=260,
    ymin=0.25, ymax=0.60,
    xtick={20,50,100,150,200,250},
    grid=major,
    grid style={gray!30},
    tick label style={font=\small},
    label style={font=\small},
    title={\small (b) Silhouette Score},
]
\addplot[color=clrRandom, mark=square*, thick, mark size=2pt]
    coordinates {(20,0.344)(30,0.328)(35,0.365)(40,0.411)
                 (45,0.379)(50,0.399)(100,0.341)(250,0.385)};
\addplot[color=clrTabu, mark=triangle*, thick, mark size=2pt]
    coordinates {(20,0.351)(30,0.287)(35,0.327)(40,0.297)
                 (45,0.390)(50,0.386)(100,0.320)(250,0.384)};
\addplot[color=clrSim, mark=diamond*, thick, mark size=2pt]
    coordinates {(20,0.351)(30,0.303)(35,0.365)(40,0.297)
                 (45,0.390)(50,0.386)(100,0.341)(250,0.384)};
\addplot[color=clrHybrid, mark=pentagon*, thick, mark size=2pt]
    coordinates {(20,0.351)(30,0.287)(35,0.345)(40,0.297)
                 (45,0.390)(50,0.386)(100,0.344)(250,0.385)};
\addplot[color=clrKpp, mark=o, thick, dashed, mark size=2pt]
    coordinates {(20,0.544)(30,0.489)(35,0.501)(40,0.556)
                 (45,0.511)(50,0.545)(100,0.454)(250,0.502)};
\end{axis}
\end{tikzpicture}
\end{subfigure}

\vspace{2pt}
\centering
\begin{tikzpicture}
\begin{axis}[
    hide axis,
    xmin=0, xmax=1, ymin=0, ymax=1,
    legend columns=5,
    legend style={draw=gray!50, font=\small, column sep=6pt,
                  anchor=center, at={(0.5,0.5)}},
    scale only axis, width=0.01cm, height=0.01cm,
]
\addlegendimage{color=clrRandom, mark=square*, thick, mark size=2pt}
\addlegendentry{Random}
\addlegendimage{color=clrTabu, mark=triangle*, thick, mark size=2pt}
\addlegendentry{TABU}
\addlegendimage{color=clrSim, mark=diamond*, thick, mark size=2pt}
\addlegendentry{SimAnn}
\addlegendimage{color=clrHybrid, mark=pentagon*, thick, mark size=2pt}
\addlegendentry{Hybrid}
\addlegendimage{color=clrKpp, mark=o, thick, dashed, mark size=2pt}
\addlegendentry{$k$-means++}
\end{axis}
\end{tikzpicture}

\caption{Clustering performance on Gaussian blob data. (a) V-measure
and (b) silhouette score across initialization methods. $k$-means++
substantially outperforms all other methods at every sample size.}
\label{fig:gaussian}
\end{figure}
\FloatBarrier

